Compositionality of Approximate Bisimulation for Probabilistic Systems

Probabilistic transition system specifications using the rule format ntmuft-ntmuxt provide structural operational semantics for Segala-type systems and guarantee that probabilistic bisimilarity is a congruence. Probabilistic bisimilarity is for many applications too sensitive to the exact probabilities of transitions. Approximate bisimulation provides a robust semantics that is stable with respect to implementation and measurement errors of probabilistic behavior. We provide a general method to quantify how much a process combinator expands the approximate bisimulation distance. As a direct application we derive an appropriate rule format that guarantees compositionality with respect to approximate bisimilarity. Moreover, we describe how specification formats for non-standard compositionality requirements may be derived.

==> eptcsdata.tex <==
\providecommand{\firstpage}{32}
\providecommand{\publicationstatus}{J. Borgstr\"om and B. Luttik (Eds.): Combined Workshop on\\
Expressiveness in Concurrency and Structural Operational\\
Semantics (EXPRESS/SOS 2013)\\
EPTCS 120, 2013, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.120.4}{10.4204/EPTCS.120.4}}
\pdfoutput=1

